A Fully Coupled Immersed Finite Element Method for Fluid Structure Interaction via the Deal.II Library

We present the implementation of a solution scheme for fluid-structure interaction problems via the finite element software library deal.II. The solution scheme is an immersed finite element method in which two independent discretizations are used for the fluid and immersed deformable body. In this type of formulation the support of the equations of motion of the fluid is extended to cover the union of the solid and fluid domains. The equations of motion over the extended solution domain govern the flow of a fluid under the action of a body force field. This body force field informs the fluid of the presence of the immersed solid. The velocity field of the immersed solid is the restriction over the immersed domain of the velocity field in the extended equations of motion. The focus of this paper is to show how the determination of the motion of the immersed domain is carried out in practice. We show that our implementation is general, that is, it is not dependent on a specific choice of the finite element spaces over the immersed solid and the extended fluid domains. We present some preliminary results concerning the accuracy of the proposed method.

==> figures/current_configuration/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
% ***** YOUR FIGURE LABELS GO BELOW *****

$\Omega$ $B_{t}$ $P$ $\bv{x}_{P}(t)$ $O$
\end{document}

==> figures/integration/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
% ***** YOUR FIGURE LABELS GO BELOW *****

fluid cell \textsf{A}

fluid cell \textsf{B}

fluid cell \textsf{C}

fluid cell \textsf{D}

solid cell

$\bullet$: quadrature point of the solid cell
\end{document}

==> figures/jumps/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
% ***** YOUR FIGURE LABELS GO BELOW *****

$\Omega$ $B_{t}$

$\bv{n}$ $\bv{\nu}^{+}$ $\bv{\nu}^{-}$

$\mathscr{D}^{+}$ $\mathscr{D}^{-}$

$\mathscr{S}_{t}$

\end{document}

==> figures/ldcflow_ball_geometry/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
% ***** YOUR FIGURE LABELS GO BELOW *****
$x$
%
\hskip 1in
%
$y$
%
\vskip 0.5in
%
$R$
\hskip 1in
$l$
%
\vskip 0.5in
$O$
%
\hskip 1in
$C$
%
\vskip 0.5in
%
$B_{t}$
%
\hskip 1in
%
$\Omega$
%
\vskip 0.5in
%
$U$
\end{document}

==> figures/ring_eqm_geometry/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
% ***** YOUR FIGURE LABELS GO BELOW *****

$\hat{\bv{u}}_{\Theta}$,
%
$\hat{\bv{u}}_{\theta}$
%
\vskip 0.5in
%
$\hat{\bv{u}}_{R}$,
%
$\hat{\bv{u}}_{r}$
%
\vskip 0.5in
%
$\Theta$,
%
$\theta$
%
\vskip 0.5in
%
$x$
%
\vskip 0.5in
%
$y$
%
\vskip 0.5in
%
$R$
\hskip 1in
$w$
\hskip 1in
$l$
%
\vskip 0.5in
%
$l/2$
%
\hskip 1in
%
$O$
%
\hskip 1in
$C$
%
\vskip 0.5in
%
$B$, $B_{t}$
%
\hskip 1in
%
$\Omega$
\end{document}

==> figures/ring_eqm_pressure/labels.tex <==
\input{../../class_packages_commands}
\newcommand{\fontlabelsizeswitch}{\small}

\begin{document}
\thispagestyle{empty}
\fontlabelsizeswitch
\setlength{\parindent}{0cm} 
% ***** YOUR FIGURE LABELS GO BELOW *****
$0.2$ \hskip0.2in 
$0.4$ \hskip0.2in
$0.6$ \hskip0.2in
$0.8$ \hskip0.2in
$1.0$ \hskip0.2in
\vskip1in
$0.2000$ \vskip0.1in
$0.1325$ \vskip0.1in
$0.0650$ \vskip0.1in
$-0.0025$ \vskip0.1in
$-0.0700$ \vskip0.1in
\vskip1in
Max: $0.1768$ \\
Min: $-0.06303$ \\ \\
Max: $0.1716$ \\
Min: $-0.05787$ 
\vskip1in
$x (m)$ \\
$y (m)$ \\
\vskip1in
Pressure
\end{document}
